Parallel Algorithms and Heuristics for Efficient Computation of High-Order Line Graphs of Hypergraphs

This paper considers structures of systems beyond dyadic (pairwise) interactions and investigates mathematical modeling of multi-way interactions and connections as hypergraphs, where captured relationships among system entities are set-valued. To date, in most situations, entities in a hypergraph are considered connected as long as there is at least one common "neighbor". However, minimal commonality sometimes discards the "strength" of connections and interactions among groups. To this end, considering the "width" of a connection, referred to as the $s$-overlap of neighbors, provides more meaningful insights into how closely the communities or entities interact with each other. In addition, $s$-overlap computation is the fundamental kernel to construct the line graph of a hypergraph, a low-order approximation of the hypergraph which can carry significant information about the original hypergraph. Subsequent stages of a data analytics pipeline then can apply highly-tuned graph algorithms on the line graph to reveal important features. Given a hypergraph, computing the $s$-overlaps by exhaustively considering all pairwise entities can be computationally prohibitive. To tackle this challenge, we develop efficient algorithms to compute $s$-overlaps and the corresponding line graph of a hypergraph. We propose several heuristics to avoid execution of redundant work and improve performance of the $s$-overlap computation. Our parallel algorithm, combined with these heuristics, is orders of magnitude (more than $10\times$) faster than the naive algorithm in all cases and the SpGEMM algorithm with filtration in most cases (especially with large $s$ value).

==> TODO.tex <==
7. update figure 2? with the figure from Andrew's example in Omnigraffle
15. Replace figure 2 with Andrew's figure.
19. To the best of knowledge, we compare with Hypernetx, which is the only available impl of the soverlap computation. HypernetX is a python module that does hypergraph analysis. We use HypernetX (which uses NetworkX to do the soverlap computation, mention the version on Github) to compute soverlap of our smallest dataset -- DNS001 (#number of nodes, #number of edges), which could not finish the computation in more than several hours. 
20. Somehow emphasize the computation is too expensive with naive algo since the time complexity is O(n3), matrix matrix multiplication
21. run Vtune : relabel by degree in ascending order is better due to cache-friendliness of the algorithms
22. Pull in changes from the ACDA paper about the linear algebra formulation.
23. Table 2 and other figure legends: change f\_x to meaningful names.
24. References: find alternative to arxiv reference for Cliff's papers??


1. cut short any discussion about graphs, s-walk
2. New table showing computational intensiveness
3. SpGEMM comparison plot in line graph in results section
4. Motivation
5. Example demonstrating application of s-line graph.
6. Put 3.6 before 3.3 (discuss SpGEMM and filter here).
7.  Even with large s value (s=1024 for example with Friendster), we have large number of s-connected components (for example 20 of them ). That means still large s values make sense and they signify tightly interconnected communities. Need t o mention this in the context of Friendster, where we keep increasing the size of s for comparing against SpGEMM.
8. Forward reference SpGEMM in the linear algebraic formulation.
9. Get more application of s line graph
10. Fix numbering in Fig 1
11. We don't have to do it immediately but we have to make sure that the x and y axis labels /values are big enough to read> For example, Fig 11, even with zooming in, the numbers are not very readable. Also the legends can be merged into one.
12. Can line numbers be added?

